Computing Large-Scale Matrix and Tensor Decomposition with Structured Factors: A Unified Nonconvex Optimization Perspective

The proposed article aims at offering a comprehensive tutorial for the computational aspects of structured matrix and tensor factorization. Unlike existing tutorials that mainly focus on {\it algorithmic procedures} for a small set of problems, e.g., nonnegativity or sparsity-constrained factorization, we take a {\it top-down} approach: we start with general optimization theory (e.g., inexact and accelerated block coordinate descent, stochastic optimization, and Gauss-Newton methods) that covers a wide range of factorization problems with diverse constraints and regularization terms of engineering interest. Then, we go `under the hood' to showcase specific algorithm design under these introduced principles. We pay a particular attention to recent algorithmic developments in structured tensor and matrix factorization (e.g., random sketching and adaptive step size based stochastic optimization and structure-exploiting second-order algorithms), which are the state of the art---yet much less touched upon in the literature compared to {\it block coordinate descent} (BCD)-based methods. We expect that the article to have an educational values in the field of structured factorization and hope to stimulate more research in this important and exciting direction.

==> gn-system.tex <==
\definecolor{kulblue}{RGB}{0,85,165}
\pgfdeclareverticalshading{diagonal}{100bp}{%
  color(0bp)=(minimal axis color!20!white);
  color(48bp)=(minimal axis color!20!white);
  color(49bp)=(red!60!black);
  color(51bp)=(red!60!black);
  color(52bp)=(minimal axis color!20!white);
  color(100bp)=(minimal axis color!20!white)}

  \colorlet{accentcolor}{kulblue!60!black}
  \colorlet{colorone}{blue!60!black}
  \colorlet{colortwo}{green!60!black}
  \colorlet{colorthree}{red!60!black}
  
  \begin{tikzpicture}[%
    text=minimal axis color,
    font=\footnotesize,
    line width=0.5pt,
    draw=minimal axis color,
    mygray/.style={minimal axis color},
    all tensors/.append style={2d,tensor scale=0.6},
    hblock/.append style={frontal matrix, dim={1,1}, anchor=A},
    xblock/.append style={frontal matrix, dim={1,0.2}, anchor=A},
    myarrow/.append style={->,shorten >=2pt,shorten <=2pt, >=stealth,mygray},
    fillaccent/.append style={fill=accentcolor,draw=white},
    fillthree/.append style={fill=colorthree,draw=white},
    subdued/.append style={fill=minimal axis color!20!white,draw=white},
    diag/.append style={shading=diagonal,shading angle=-45,draw=white},
    node distance=0.8cm]

    \node [frontal matrix, dim={3,3},subdued] (J1T) {};
    \node at (J1T.1 1) [hblock,diag] (h11) {};
    \node at (J1T.1 2) [hblock,diag] (h12) {};
    \node at (J1T.1 3) [hblock,subdued] (h13) {};
    \node at (J1T.2 1) [hblock,subdued] (h21) {};
    \node at (J1T.2 2) [hblock,subdued] (h22) {};
    \node at (J1T.2 3) [hblock,diag] (j1tc) {};
    \node at (J1T.3 1) [hblock,subdued] (h31) {};
    \node at (J1T.3 2) [hblock,subdued] (h32) {};
    \node at (J1T.3 3) [hblock,subdued] (h33) {};

    \node [frontal matrix, dim={3,3},subdued,right=1mm of J1T] (H1) {};
    \node at (H1.1 1) [hblock,fillaccent] (h11) {};
    \node at (H1.1 2) [hblock,fillaccent] (h12) {};
    \node at (H1.1 3) [hblock,fillaccent] (h13) {};
    \node at (H1.2 1) [hblock,fillaccent] (h21) {};
    \node at (H1.2 2) [hblock,fillaccent] (h22) {};
    \node at (H1.2 3) [hblock,fillaccent] (h23) {};
    \node at (H1.3 1) [hblock,fillaccent] (h31) {};
    \node at (H1.3 2) [hblock,fillaccent] (h32) {};
    \node at (H1.3 3) [hblock,fillaccent] (h33) {};

    \node [frontal matrix, dim={3,3},subdued,right=1mm of H1] (J1) {};
    \node at (J1.1 1) [hblock,diag] (h11) {};
    \node at (J1.1 2) [hblock,subdued] (h12) {};
    \node at (J1.1 3) [hblock,subdued] (h13) {};
    \node at (J1.2 1) [hblock,diag] (h21) {};
    \node at (J1.2 2) [hblock,subdued] (h22) {};
    \node at (J1.2 3) [hblock,subdued] (h23) {};
    \node at (J1.3 1) [hblock,subdued] (h31) {};
    \node at (J1.3 2) [hblock,diag] (j1c) {};
    \node at (J1.3 3) [hblock,subdued] (h33) {};

    \node [frontal matrix, dim={3,2},subdued, right=of J1] (J2T) {};
    \node at (J2T.1 1) [hblock,subdued] (h21) {};
    \node at (J2T.1 2) [hblock,subdued] (h22) {};
    \node at (J2T.2 1) [hblock,diag] (j2tc) {};
    \node at (J2T.2 2) [hblock,subdued] (h22) {};
    \node at (J2T.3 1) [hblock,subdued] (h31) {};
    \node at (J2T.3 2) [hblock,fillthree,] (h32t) {};

    \node at (J2T.C) [frontal matrix, dim={2,2},subdued,xshift=1mm,anchor=A] (H2) {};
    \node at (H2.1 1) [hblock,fillaccent] (h21) {};
    \node at (H2.1 2) [hblock,fillaccent] (h22) {};
    \node at (H2.2 1) [hblock,fillaccent] (h21) {};
    \node at (H2.2 2) [hblock,fillaccent] (h22) {};

    \node [frontal matrix, dim={2,3},subdued, right=1mm of H2] (J2) {};
    \node at (J2.1 1) [hblock,subdued] (h21) {};
    \node at (J2.1 2) [hblock,diag] (j2c) {};
    \node at (J2.1 3) [hblock,subdued] (h21) {};
    \node at (J2.2 1) [hblock,subdued] (h22) {};
    \node at (J2.2 2) [hblock,subdued] (h31) {};
    \node at (J2.2 3) [hblock,fillthree] (h32) {};

    \node at ($(J1.east)!0.5!(J2T.west)$) (plus1) {$+$};

    %% Annotations
    \draw [rounded corners=1pt,colortwo]
    ($(J1T.1 1)+(-0.5mm,0.5mm)$) rectangle
    ($(J1T.2 3)+(0.5mm,-0.5mm)$);
    \draw [rounded corners=1pt,colortwo]
    ($(J1.1 1)+(-0.5mm,0.5mm)$) rectangle
    ($(J1.3 2)+(0.5mm,-0.5mm)$);

    \node at (H1) [yshift=14mm,xshift=-5mm,colortwo] (sym) {symmetry};
    \draw [myarrow,->,shorten >=1mm,colortwo] (sym.west) to [bend right] (J1T.1 2);
    %\draw [myarrow,->,shorten >=1mm,colortwo] (sym.east) to [bend left]  ($(J1.1 1)!0.5!(J1.1 2)$);

    \node at ($(h32t.B)!0.5!(h32t.D)$) [yshift=-4mm,xshift=3mm,colorthree,anchor=west] (param)
    {parametric};
    \draw [myarrow,<-,shorten <=1mm,colorthree] ($(h32t.B)!0.5!(h32t.D)$) to
    [bend right] (param.west);

    \draw [rounded corners=1pt,mygray,densely dotted]
    ($(J2T.2 1)+(-0.5mm,-0.5mm)$) rectangle
    ($(J2T.C)+(0.5mm,0.5mm)$);
    \draw [rounded corners=1pt,mygray,densely dotted]
    ($(J2.B)+(-0.5mm,-0.5mm)$) rectangle
    ($(J2.1 2)+(0.5mm,0.5mm)$);
    
    \draw [rounded corners=1pt,mygray,densely dotted]
    ($(J1T.3 1)+(-0.5mm,0.5mm)$) rectangle
    ($(J1T.D)+(0.5mm,-0.5mm)$);
    \draw [rounded corners=1pt,mygray,densely dotted]
    ($(J1.1 3)+(-0.5mm,0.5mm)$) rectangle
    ($(J1.D)+(0.5mm,-0.5mm)$);
    
    \node at (H1) [yshift=-14mm,xshift=5mm,mygray] (unused) {unused variable};
    %\draw [myarrow,->,shorten >=1mm] (unused.west) to [bend left] ($(J1T.B)!0.5!(J1T.D)$);
    \draw [myarrow,->,shorten >=1mm] (unused.east) to [bend right]  ($(J1.B)!0.83!(J1.D)$);

    \draw [rounded corners=1pt,colorone,dashed]
    ($(j1tc.A)+(-0.5mm,0.5mm)$) rectangle
    ($(j1tc.D)+(0.5mm,-0.5mm)$);
    \draw [rounded corners=1pt,colorone,dashed]
    ($(j1c.A)+(-0.5mm,0.5mm)$) rectangle
    ($(j1c.D)+(0.5mm,-0.5mm)$);
    \draw [rounded corners=1pt,colorone,dashed]
    ($(j2tc.A)+(-0.5mm,0.5mm)$) rectangle
    ($(j2tc.D)+(0.5mm,-0.5mm)$);
    \draw [rounded corners=1pt,colorone,dashed]
    ($(j2c.A)+(-0.5mm,0.5mm)$) rectangle
    ($(j2c.D)+(0.5mm,-0.5mm)$);

    \node at ($(j2c.A)!0.5!(j2c.C)$) [yshift=4mm,xshift=-3mm,accentcolor,anchor=east,colorone] (coupled)
    {coupling};
    \draw [myarrow,<-,shorten <=1mm,colorone] ($(j2c.A)!0.5!(j2c.C)$) to [bend right] (coupled.east);
    
    % Parenthesis
    \draw [] ($(J1T.B)+(-2mm,-2mm)$) to [bend left=10] ($(J1T.A)+(-2mm,2mm)$);
    \draw [] ($(J2.D|-J2T.D)+(2mm,-2mm)$) to [bend right=10] ($(J2.C)+(2mm,2mm)$);

    % X vector 
    \node at ($(J2T.east-|J2.east)$) [frontal matrix, dim={3,0.2},anchor=west,subdued,xshift=6mm] (X) {};
    \node at (X.1 1) [xblock,fillaccent] (x1) {};
    \node at (X.2 1) [xblock,fillaccent] (x2) {};
    \node at (X.3 1) [xblock,fillaccent] (x3) {};
    
    \node at ($(J2.east|-J2T.east)!0.5!(X.west)$) [xshift=1.5mm] (dot) {$\cdot$};

    \node [frontal matrix, dim={3,3},subdued,right=8mm of X] (J1T) {};
    \node at (J1T.1 1) [hblock,diag] (h11) {};
    \node at (J1T.1 2) [hblock,diag] (h12) {};
    \node at (J1T.1 3) [hblock,subdued] (h13) {};
    \node at (J1T.2 1) [hblock,subdued] (h21) {};
    \node at (J1T.2 2) [hblock,subdued] (h22) {};
    \node at (J1T.2 3) [hblock,diag] (h23) {};
    \node at (J1T.3 1) [hblock,subdued] (h31) {};
    \node at (J1T.3 2) [hblock,subdued] (h32) {};
    \node at (J1T.3 3) [hblock,subdued] (h33) {};

    \node [frontal matrix, dim={3,0.2},right=1mm of J1T,subdued] (G1) {};
    \node at (G1.1 1) [xblock,fillaccent] (g1) {};
    \node at (G1.2 1) [xblock,fillaccent] (g2) {};
    \node at (G1.3 1) [xblock,fillaccent] (g3) {};

    \node [frontal matrix, dim={3,2},subdued, right=4mm of G1] (J2T) {};
    \node at (J2T.1 1) [hblock,subdued] (h21) {};
    \node at (J2T.1 2) [hblock,subdued] (h22) {};
    \node at (J2T.2 1) [hblock,diag] (h21) {};
    \node at (J2T.2 2) [hblock,subdued] (h22) {};
    \node at (J2T.3 1) [hblock,subdued] (h31) {};
    \node at (J2T.3 2) [hblock,fillthree] (h32) {};

    \node at (J2T.C) [frontal matrix, dim={2,0.2},anchor=A,xshift=1mm,subdued] (G2) {};
    \node at (G2.1 1) [xblock,fillaccent] (g1) {};
    \node at (G2.2 1) [xblock,fillaccent] (g2) {};

    \node at ($(G1.east)!0.5!(J2T.west)$) (plus2) {$+$};

    % Parenthesis
    \draw [mygray] ($(J1T.B)+(-2mm,-2mm)$) to [bend left=10] ($(J1T.A)+(-2mm,2mm)$);
    \draw [mygray] ($(G2.D|-J2T.D)+(2mm,-2mm)$) to [bend right=10] ($(G2.C)+(2mm,2mm)$);
    
    \node at ($(X.east)!0.5!(J1T.west)$) [xshift=-1.5mm] (eq) {$=$};

    % Text nodes 
    \node at (H1) [yshift=-2cm] (tmp) {$\lambda_1\tilde{\mat{J}}_1^{\T}\cdot\bm{\varPhi}_1\cdot\tilde{\mat{J}}_1$};
    \node at (tmp) [xshift=-16mm] {$($};
    \node at (plus1|-tmp) {$+$};
    \node at (H2|-tmp) (h2l) {$\lambda_2\tilde{\mat{J}}_{2}^{\T}\cdot\bm{\varPhi}_2\cdot\tilde{\mat{J}}_2$};
    \node at (h2l) [xshift=16mm] (tmp) {$)$};
    \node at (dot|-tmp) {$\cdot$};
    \node at (X|-tmp) {$\vec{p}$};
    \node at (eq|-tmp) {$=$};
    \node at (J1T|-tmp) (g1l) {$-\lambda_1\tilde{\mat{J}}_1^{\T}\cdot\vec{g}_1$};
    \node at (g1l) [xshift=-9mm] {$($};
%    \node at (plus2|-tmp) [xshift=-1mm] {$-$};
    \node at (J2T|-tmp) (g2l) {$-\lambda_2\tilde{\mat{J}}_2^{\T}\cdot\vec{g}_2$};
    \node at (g2l) [xshift=9mm] {$)$};

    % Extra explanation
    \draw [myarrow] ($(h11.A)!0.5!(h11.C)$) to [out=80, in=-20] ++(-4mm,5mm) node
    [anchor=east,inner sep=1pt] {$\mat{I}$}; 
    \draw [myarrow] ($(h13.A)!0.5!(h13.C)$) to [out=80, in=-170] ++(7mm,5mm) node
    [anchor=west,inner sep=1pt] {$\mat{0}$}; 
    
  \end{tikzpicture}

